CoCoAFusE: Beyond Mixtures of Experts via Model Fusion

Many learning problems involve multiple patterns and varying degrees of uncertainty dependent on the covariates. Advances in Deep Learning (DL) have addressed these issues by learning highly nonlinear input-output dependencies. However, model interpretability and Uncertainty Quantification (UQ) have often straggled behind. In this context, we introduce the Competitive/Collaborative Fusion of Experts (CoCoAFusE), a novel, Bayesian Covariates-Dependent Modeling technique. CoCoAFusE builds on the very philosophy behind Mixtures of Experts (MoEs), blending predictions from several simple sub-models (or "experts") to achieve high levels of expressiveness while retaining a substantial degree of local interpretability. Our formulation extends that of a classical Mixture of Experts by contemplating the fusion of the experts' distributions in addition to their more usual mixing (i.e., superimposition). Through this additional feature, CoCoAFusE better accommodates different scenarios for the intermediate behavior between generating mechanisms, resulting in tighter credible bounds on the response variable. Indeed, only resorting to mixing, as in classical MoEs, may lead to multimodality artifacts, especially over smooth transitions. Instead, CoCoAFusE can avoid these artifacts even under the same structure and priors for the experts, leading to greater expressiveness and flexibility in modeling. This new approach is showcased extensively on a suite of motivating numerical examples and a collection of real-data ones, demonstrating its efficacy in tackling complex regression problems where uncertainty is a key quantity of interest.

==> Figures/switch/results.tex <==
\begin{tabular}{lccccc}
	% table generated automatically on date 2025-01-31
	\toprule
	& Train & \multicolumn{4}{c}{Test} \\

	\cmidrule(lr){2-2}\cmidrule(lr){3-6}
	& $\uparrow$ LOO
	& $\uparrow$ LPPD
	& $_\uparrow^\downarrow$ 95\% CIC
	& $\downarrow$ 95\% CIL
	& $\downarrow$ eMSE \\

	\midrule

	% data extracted automatically on date 2025-01-31 from path outputs/transition/moe/inference/evaluation.csv
	MoE3 &
		-144.99\textpm19.53 &
		-112.49\textpm14.45 &
		0.97\textpm0.01 &
		1.40\textpm0.02 &
		0.24\textpm0.01\\

	% data extracted automatically on date 2025-01-31 from path outputs/transition/moe2ex/inference/evaluation.csv
	MoE2 &
		-400.22\textpm21.95 &
		-415.83\textpm21.86 &
		0.98\textpm0.01 &
		2.12\textpm0.04 &
		0.58\textpm0.03\\

	% data extracted automatically on date 2025-01-31 from path outputs/transition/boe/inference/evaluation.csv
	BoE &
		-141.10\textpm22.15 &
		-104.30\textpm15.37 &
		0.96\textpm0.01 &
		1.21\textpm0.00 &
		0.19\textpm0.01\\

	% data extracted automatically on date 2025-01-31 from path outputs/transition/cocoafuse/inference/evaluation.csv
	CoCoAFusE &
		-113.61\textpm17.70 &
		-97.81\textpm14.71 &
		0.96\textpm0.01 &
		1.22\textpm0.01 &
		0.19\textpm0.01\\

	\bottomrule
\end{tabular}
